SuperShaper: Task-Agnostic Super Pre-training of BERT Models with Variable Hidden Dimensions

Task-agnostic pre-training followed by task-specific fine-tuning is a default approach to train NLU models. Such models need to be deployed on devices across the cloud and the edge with varying resource and accuracy constraints. For a given task, repeating pre-training and fine-tuning across tens of devices is prohibitively expensive. We propose SuperShaper, a task agnostic pre-training approach which simultaneously pre-trains a large number of Transformer models by varying shapes, i.e., by varying the hidden dimensions across layers. This is enabled by a backbone network with linear bottleneck matrices around each Transformer layer which are sliced to generate differently shaped sub-networks. In spite of its simple design space and efficient implementation, SuperShaper discovers networks that effectively trade-off accuracy and model size: Discovered networks are more accurate than a range of hand-crafted and automatically searched networks on GLUE benchmarks. Further, we find two critical advantages of shape as a design variable for Neural Architecture Search (NAS): (a) heuristics of good shapes can be derived and networks found with these heuristics match and even improve on carefully searched networks across a range of parameter counts, and (b) the latency of networks across multiple CPUs and GPUs are insensitive to the shape and thus enable device-agnostic search. In summary, SuperShaper radically simplifies NAS for language models and discovers networks that generalize across tasks, parameter constraints, and devices.

==> Images/shape_perplexity_correlation_table.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrrr}\toprule
\textbf{Evo-search parameters} &\textbf{G\_Direct} &\textbf{Parameter range} &\textbf{Num networks} &\textbf{Spearman correlation} &\textbf{Pearson correlation} \\\cmidrule{1-6}
53 &8.59 &52-54 &54 &71.03 &67.95 \\\cmidrule{1-6}
63 &7.09 &62-64 &704 &80.34 &82.52 \\\cmidrule{1-6}
65 &6.86 &63-65 &862 &69.47 &71.34 \\\cmidrule{1-6}
69 &6.62 &68-70 &1065 &47.22 &52.06 \\\cmidrule{1-6}
80 &6.17 &79-81 &486 &72.32 &67.34 \\\cmidrule{1-6}
90.5 &5.83 &89-91 &47 &56.8 &54.67 \\\cmidrule{1-6}
96 &5.65 &95-97 &6 &65.71 &69.65 \\\midrule
\bottomrule
\caption{Caption}\label{tab: }
\end{tabular}
\end{table}
